RADARSAT Constellation Mission Compact Polarisation SAR Data for Burned Area Mapping with Deep Learning

Monitoring wildfires has become increasingly critical due to the sharp rise in wildfire incidents in recent years. Optical satellites like Sentinel-2 and Landsat are extensively utilized for mapping burned areas. However, the effectiveness of optical sensors is compromised by clouds and smoke, which obstruct the detection of burned areas. Thus, satellites equipped with Synthetic Aperture Radar (SAR), such as dual-polarization Sentinel-1 and quad-polarization RADARSAT-1/-2 C-band SAR, which can penetrate clouds and smoke, are investigated for mapping burned areas. However, there is limited research on using compact polarisation (compact-pol) C-band RADARSAT Constellation Mission (RCM) SAR data for this purpose. This study aims to investigate the capacity of compact polarisation RCM data for burned area mapping through deep learning. Compact-pol m-chi decomposition and Compact-pol Radar Vegetation Index (CpRVI) are derived from the RCM Multi-look Complex product. A deep-learning-based processing pipeline incorporating ConvNet-based and Transformer-based models is applied for burned area mapping, with three different input settings: using only log-ratio dual-polarization intensity images images, using only compact-pol decomposition plus CpRVI, and using all three data sources. The results demonstrate that compact-pol m-chi decomposition and CpRVI images significantly complement log-ratio images for burned area mapping. The best-performing Transformer-based model, UNETR, trained with log-ratio, m-chi decomposition, and CpRVI data, achieved an F1 Score of 0.718 and an IoU Score of 0.565, showing a notable improvement compared to the same model trained using only log-ratio images.

==> highlights.tex <==
\begin{highlights}

\item 1) Demonstrating the compact-pol m-$\chi$ decomposition and compact-pol vegetation index images, generated from RCM C-band Multilook Complex product, complement the log-ratio intensity images effectively for burned area mapping.

\item 2) Combining compact-pol RCM data with ConvNet-based and Transformer-based segmentation models, the proposed workflow can effectively detect wildfires in 7 study regions at 9 timestamps in the test dataset. The Transformer-based model UNETR provides the best F1 Score of 0.718 and IoU Score of 0.565 among other baseline models.
\end{highlights}



